Safety Monitoring for Learning-Enabled Cyber-Physical Systems in Out-of-Distribution Scenarios

The safety of learning-enabled cyber-physical systems is compromised by the well-known vulnerabilities of deep neural networks to out-of-distribution (OOD) inputs. Existing literature has sought to monitor the safety of such systems by detecting OOD data. However, such approaches have limited utility, as the presence of an OOD input does not necessarily imply the violation of a desired safety property. We instead propose to directly monitor safety in a manner that is itself robust to OOD data. To this end, we predict violations of signal temporal logic safety specifications based on predicted future trajectories. Our safety monitor additionally uses a novel combination of adaptive conformal prediction and incremental learning. The former obtains probabilistic prediction guarantees even on OOD data, and the latter prevents overly conservative predictions. We evaluate the efficacy of the proposed approach in two case studies on safety monitoring: 1) predicting collisions of an F1Tenth car with static obstacles, and 2) predicting collisions of a race car with multiple dynamic obstacles. We find that adaptive conformal prediction obtains theoretical guarantees where other uncertainty quantification methods fail to do so. Additionally, combining adaptive conformal prediction and incremental learning for safety monitoring achieves high recall and timeliness while reducing loss in precision. We achieve these results even in OOD settings and outperform alternative methods.

==> sections/timeliness_table.tex <==
\begin{table*}[t]
\caption{Recall, precision, and timeliness of our safety monitor for the F1Tenth (top) and race car (bottom) case studies, recorded over 10 trials. For both, we evaluate the influence of uncertainty quantification and incremental learning on our safety monitoring task in both the in-distribution (ID) and four out-of-distribution scenarios. For the F1Tenth case study, the OOD scenarios are 3 missing LIDAR rays, 5 missing LIDAR rays, additive uniform (0,0.9) noise, and additive uniform (0,1.0) noise. For the race car case study, the OOD scenarios are 2, 3, 4, and 5 dynamic obstacles (obs.) on the race track. Overall, both uncertainty quantification and incremental learning are necessary for safety monitoring in OOD scenarios. \label{tab:both_results}}
\centering
     \begin{minipage}[t]{0.48\linewidth}\centering
         \begin{tabular}{|c|c|cc|}
         \hline
         \multicolumn{4}{|c|}{\textbf{Case Study I}}\\
         \hline\hline
         \multirow{2}{*}{\textbf{Setting}} & \multirow{2}{*}{\textbf{UQ}} & \multicolumn{2}{|c|}{\textbf{Timeliness}}\\ [0.5ex]
         & & w/o IL & w/ IL \\
         \hline
         \multirow{4}{*}{ID} & PP & x.xx $\pm$ x.xx & -\\
                             & CP & & \\
                             & RCP & & \\
                             & ACP & & \\
        \hline
        \multirow{4}{*}{3 rays} & PP & x.xx $\pm$ x.xx & x.xx $\pm$ x.xx \\
                             & CP & &\\
                             & RCP & & \\
                             & ACP & & \\
        \hline
        \multirow{4}{*}{5 rays} & PP & x.xx $\pm$ x.xx & x.xx $\pm$ x.xx \\
                             & CP & &\\
                             & RCP & & \\
                             & ACP & & \\
        \hline
        \multirow{4}{*}{noise (0.9)} & PP &x.xx $\pm$ x.xx & x.xx $\pm$ x.xx\\
                             & CP & & \\
                             & RCP & & \\
                             & ACP & & \\
        \hline
        \multirow{4}{*}{noise (1.0)} & PP & x.xx $\pm$ x.xx & x.xx $\pm$ x.xx \\
                             & CP & & \\
                             & RCP & & \\
                             & ACP & & \\  [1ex] 
        \hline
        \end{tabular}
     \end{minipage}
     \hfill
     \begin{minipage}[t]{0.48\linewidth}\centering
         \begin{tabular}{|c|c|cc|}
         \hline
         \multicolumn{4}{|c|}{\textbf{Case Study I}}\\
         \hline\hline
         \multirow{2}{*}{\textbf{Setting}} & \multirow{2}{*}{\textbf{UQ}} & \multicolumn{2}{|c|}{\textbf{Timeliness}}\\ [0.5ex]
         & & w/o IL & w/ IL \\
         \hline
         \multirow{4}{*}{ID} & PP & x.xx $\pm$ x.xx & -\\
                             & CP & & \\
                             & RCP & & \\
                             & ACP & & \\
        \hline
        \multirow{4}{*}{3 rays} & PP & x.xx $\pm$ x.xx & x.xx $\pm$ x.xx \\
                             & CP & &\\
                             & RCP & & \\
                             & ACP & & \\
        \hline
        \multirow{4}{*}{5 rays} & PP & x.xx $\pm$ x.xx & x.xx $\pm$ x.xx \\
                             & CP & &\\
                             & RCP & & \\
                             & ACP & & \\
        \hline
        \multirow{4}{*}{noise (0.9)} & PP &x.xx $\pm$ x.xx & x.xx $\pm$ x.xx\\
                             & CP & & \\
                             & RCP & & \\
                             & ACP & & \\
        \hline
        \multirow{4}{*}{noise (1.0)} & PP & x.xx $\pm$ x.xx & x.xx $\pm$ x.xx \\
                             & CP & & \\
                             & RCP & & \\
                             & ACP & & \\  [1ex] 
        \hline
        \end{tabular}
    \end{minipage}
\end{table*}
